X-MEN: Guaranteed XOR-Maximum Entropy Constrained Inverse Reinforcement Learning

Inverse Reinforcement Learning (IRL) is a powerful way of learning from demonstrations. In this paper, we address IRL problems with the availability of prior knowledge that optimal policies will never violate certain constraints. Conventional approaches ignoring these constraints need many demonstrations to converge. We propose XOR-Maximum Entropy Constrained Inverse Reinforcement Learning (X-MEN), which is guaranteed to converge to the optimal policy in linear rate w.r.t. the number of learning iterations. X-MEN embeds XOR-sampling -- a provable sampling approach that transforms the #P complete sampling problem into queries to NP oracles -- into the framework of maximum entropy IRL. X-MEN also guarantees the learned policy will never generate trajectories that violate constraints. Empirical results in navigation demonstrate that X-MEN converges faster to the optimal policies compared to baseline approaches and always generates trajectories that satisfy multi-state combinatorial constraints.

==> tex/analysis.tex <==







==> tex/copyandpaste.tex <==
Reinforcement learning  can acquire complex behaviors from high-level specifications. However,
defining a cost function that can be optimized
effectively and encodes the correct task is challenging in practice.

and  We can then estimate the second term of equation \ref{eq:grad_ll} by sampling from $Q$. For the following parts we let the reward function $R_{\theta}(\tau)$ represented by a linear combination of hand-crafted features for simplicity, i.e., $R_{\theta}(\tau)=\theta^Tf(\tau)$, and then the sample distribution $Q$ share weights with nominal distribution $P$, i.e.,  Notice that it is not hard to extend $R_{\theta}(\tau)$ to deep neural network representation and update $\hat{\theta}$ adaptively. We leave this discussion to the supplementary materials.


\subsection{Valid trajectories generation via XOR-Sampling}

In X-MEN, we use XOR-Sampling \cite{ermon2013embed} to get samples from $Q(\tau|\hat{\theta})$,
which leverages recent advancements in sampling via hashing and randomization. In particular, this sampling scheme guarantees that the probability of drawing a sample is sandwiched between a constant bound of the true probability. 
%
We only present the general idea of XOR-Sampling on unweighted functions
here and refer the readers to the paper \cite{ermon2013embed}
for the weighted case. Notice that XOR-Sampling can directly draw samples from unnormalized distributions without the knowledge of the partition function $Z_{\hat{\theta}}$.
%
For the unweighted case, assuming $w(\tau)=I_C(\tau)e^{-\hat{\theta}^Tf(\tau)}$ takes binary values, we need to draw samples from the set $\mathcal{W}=\{\tau: w(\tau)=1\}$ uniformly at random; i.e., suppose $|\mathcal{W}|=2^l$, then each member in $\mathcal{W}$ should have $2^{-l}$ probability to be sampled.
%
Following notations from the SAT community, we call one assignment $\tau_0$ which makes $w(\tau_0)=1$ a ``satisfying assignment''. XOR-Sampling obtains near-uniform samples by querying a NP oracle to find one satisfying assignment subject to additional randomly generated XOR constraints. 
%
Initially, the NP oracle will find one satisfying assignment subject to zero XOR constraints, albeit not at random. We then keep adding XOR constraints. 
%
We can prove that in expectation, each newly added XOR constraint rules out approximately half of the satisfying assignments at random. Therefore, if we start with $2^l$ satisfying assignments in $\mathcal{W}$, after adding $l$ XOR constraints, we will be left with only one satisfying assignment in expectation. 
%
We return this assignment as our first sample. Because we can prove that the assignments are ruled out randomly, we can guarantee that the returned assignment must be a randomly chosen one from $\mathcal{W}$ \cite{Gomes2006NearUniformSampling,Gomes2007XORCounting}. Interestingly, since $I_C(\tau)$ here is a indicator function of whether trajectory $\tau$ satisfies a set of combinatorial constraints $C(\tau)$, we can add these constraints together with those XOR constraints and solve them by Mix Integer Programming solvers like Cplex simultaneously. In addition, we also add flow constraints to ensure each samples is a valid trajectory.

For the weighted case, one needs to draw samples from an unnormalized function $w(\tau)$, i.e., the probability of getting a sample $\tau_0$, $Q(\tau_0|\hat{\theta})$ is proportional to $w(\tau)$.
%
The idea is to discretize $w(\tau)$ and  transform
the weighted problem into an unweighted one with additional variables. 
%
Our paper uses the constant approximation bounds of XOR sampling on weighted functions through the following theorem. 
%
we refer the readers to \cite{ermon2013embed,fan2021xorcd,fan2021xorsgd} for the details on the discretization scheme and the choice of the parameters of the original algorithm to reach the bound in Theorem \ref{Th:bound3}.

\begin{Th}\label{Th:bound3}\cite{ermon2013embed}~
Let $\delta>1$, $0 < \gamma < 1$, $w: \{0,1\}^n \rightarrow \mathbb{R}^+$ be an unnormalized 
probability density function. $Q(\tau|\hat{\theta}) \propto w(\tau)$ is the normalized distribution. Then, with probability at least $1-\gamma$, XOR-Sampling$(w, \delta, \gamma)$ succeeds and outputs a sample $\tau_0$ by querying $O(n\ln(\frac{n}{\gamma}))$ NP oracles. Upon success, each $\tau_0$ is produced 
with probability $Q'(\tau_0)$. 
% We must have 
% $$1/\delta Q(\tau_0|\hat{\theta}) \leq Q'(\tau_0) \leq \delta Q(\tau_0|\hat{\theta}).$$ 
% Moreover, 
Then, let $\phi:\{0,1\}^n\rightarrow\mathbb{R}^+$ be one non-negative function, then the expectation of 
one sampled $\phi(\tau)$ satisfies,
\begin{align}
    \frac{1}{\delta}\mathbb{E}_{Q}[\phi(\tau)]\leq\mathbb{E}_{Q'}[\phi(\tau)] \leq\delta\mathbb{E}_{Q}[\phi(\tau)].\label{eq:bound_eq2}
\end{align}
\end{Th}

